FITNESS: A Causal De-correlation Approach for Mitigating Bias in Machine Learning Software

Software built on top of machine learning algorithms is becoming increasingly prevalent in a variety of fields, including college admissions, healthcare, insurance, and justice. The effectiveness and efficiency of these systems heavily depend on the quality of the training datasets. Biased datasets can lead to unfair and potentially harmful outcomes, particularly in such critical decision-making systems where the allocation of resources may be affected. This can exacerbate discrimination against certain groups and cause significant social disruption. To mitigate such unfairness, a series of bias-mitigating methods are proposed. Generally, these studies improve the fairness of the trained models to a certain degree but with the expense of sacrificing the model performance. In this paper, we propose FITNESS, a bias mitigation approach via de-correlating the causal effects between sensitive features (e.g., the sex) and the label. Our key idea is that by de-correlating such effects from a causality perspective, the model would avoid making predictions based on sensitive features and thus fairness could be improved. Furthermore, FITNESS leverages multi-objective optimization to achieve a better performance-fairness trade-off. To evaluate the effectiveness, we compare FITNESS with 7 state-of-the-art methods in 8 benchmark tasks by multiple metrics. Results show that FITNESS can outperform the state-of-the-art methods on bias mitigation while preserve the model's performance: it improved the model's fairness under all the scenarios while decreased the model's performance under only 26.67% of the scenarios. Additionally, FITNESS surpasses the Fairea Baseline in 96.72% cases, outperforming all methods we compared.

==> Z_draft.tex <==

This is the age of data, this is the age of algorithms. A perfect commercial close loop has been built via data, algorithms, applications and users. The data and algorithm based applications and services enormously enriched people's life, changed people's work styles and enhanced social efficiency. Nonetheless, we should not omit the negative effect beneath the tremendous success as well. Science and technology are neutral while data and data-driven algorithms are frequently not. Affecting by biased data, algorithms exacerbate social prejudice and discrimination. The Matthew effect becomes more pronounced. Indeed, the biased data should be blamed, but actually how to process raw data is more critical for addressing the problems. We provides a new perspective to deal with bias and unreliable correlation in the dataset.
\shangwen{We do not need this paragraph. We just introduce the workflow of CUFF and draw a figure to demonstrate it.}

Nowadays, recommendation systems are widely-used in web services. Such systems are generally based on machine learning models, whose quality is evidently affected by the dataset quality    \cite{mehrabi2021survey, tsioutsiouliklis2022link, li2021user}. An ideal dataset is expected to be class-balanced, diverse, large-scale, and confound-free. 
However, in practice, the dataset is usually biased and limited in size because of the cost and privacy policy constrain \cite{mehrabi2021survey}. Imbalanced class distribution and confounds decrease the model's performance. At the same time, the bias with respect to the human sensitive features may produce prejudice and discrimination, which are likely to cause severe fairness problems and social disruption to the learned model. 

The interaction between users and web services or applications aggregates the unfairness in data and model preferences as well \cite{mehrabi2021survey}. In such scenarios as social media push and online shopping, users' clicks produce more similar data exaggerating model preferences. Though web service providers and advertisers favor these results, they put the user at a disadvantage, \ie a cocoon filled with homogeneous information, which obviously runs counter to the web spirit of openness, freedom and equality \cite{assembly1948universal, ji2020crack}. Thus,  in Web, AI, ML and SE communities, lots of work aims to address the bias and fairness problems in modern web services.

\subsection{Biased Data and Unreliable Correlation}
\shangwen{do we need this subsection in the Approach section? If you mean biased data will result in unreliable correlation, then maybe introduce these contents in Motivation?}
\shangwen{What are the logic connections among the three sub-parts here? Need more clarifications at the beginning of each sub-part.}
The dataset quality evidently affects machine learning model quality. An ideal dataset is expected to be class balanced, diverse, large enough and without confounds. However, the actual dataset is usually biased and limited in size because of the cost and privacy policy constrain. Imbalanced class distribution and confounds decrease the model's performance. At the same time, the bias locating on human sensitive features may produce prejudice and discrimination, which are likely to cause severe fairness problems and social disruption.

\subsubsection{Imbalanced Dataset}
Adult Income Dataset is a typical biased dataset with fourteen features (e.g., age, work class, education, sex, ... ) and one label (income > 50k or income <= 50k). The majority class is low income people (income <= 50k) accounting for 76\% while only 24\% instances are high income (income > 50k). Besides, the sex and race distribution are imbalanced as well. Among the high-income group, only 14\% are female while 86\% are male.

\subsubsection{Unreliable Correlation}

The mainstream machine learning algorithms are statistically fit the correlation among individual variables in the data to make predictions or decisions. However, in the real world, correlation is a ubiquitous relationship; even two unrelated things may show a strong positive or negative correlation. For example, a study \cite{} showed that nationals of countries that love chocolate are more likely to win a Nobel Prize. The author proposed three hypothesis:

1. Chocolate enhances one's cognitive abilities, which increases the probability of winning a Nobel Prize;

2. Cognitive people love chocolate, and Nobel laureates are no exception;

3. In countries with good economic conditions, people are more likely to afford to consume chocolate and have access to good education and research conditions. Then people are more likely to win a Nobel Prize.

A study [] confirmed the third hypothesis, as the number of Nobel laureates and the number of IKEA stores per population area and GDP per capita showed a similar positive correlation with chocolate consumption.

\subsubsection{Machine learning prefers shortcuts}

The innate characteristic determines that the machine learning algorithms prefer the shortest one among all the potential paths. For example, in a cattle recognition task, if all the cattle label images were with a grassland background, the learned model would predict all grassland background images as cattle pictures instead of concentrating on the original features of color, skeleton and texture of cattle. Obviously, such models aren't those we need.



\subsubsection{More Stable Model}
Although this paper focuses on the fairness problem, we obtained an extra benefit from CUFF. After causal de-correlation, the learned model performs more robust and stable in Out-of-Distribution (OOD) scenarios. \shangwen{Is there any experiment result to demonstrate this?}
It will be a direction guiding our further study.


\subsection{Benefits of De-correlation}
As the two severe problems mentioned above, we proposed a causal de-correlated method to interdict the unreliable correlation among variables to avoid the model learning them and making unreliable decisions. With causal de-correlation, we can gain at least two potential benefits: a fairer machine learning model and a more stable machine learning model.\shangwen{I am not sure if we need to mention stable here. It has not been proposed in this paper before.}

\subsubsection{Fairer Model}
Building a fair and equal society free from discrimination and prejudice is a beautiful vision for all humanity. To support this vision, machine learning engineers and scholars are devoted to making each model and algorithm fairer. Hence, fairness is a critical non-functional metric of machine learning models and software. 


\begin{table*}[htbp]
  \centering
  \caption{Table 1: Description of the dataset used in this paper}\resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|}%
    \hline
    \centering
    \rowcolor{lightgray}
    Dataset & Features & \makecell{Sensitive \\Features} & Size & Description \\
    \hline
    Adult Census Income & 14 & Sex, Race & 48842 &  Individual information from 1994 U.S. census. Goal is predicting income >\$50,000.\\
    \hline
    Compas	& 28	& Sex, Race	& 7214	& Contains criminal history of defendants. Goal predicting re-offending in future.\\
    \hline
    German Credit & 20	& Sex	& 1000	& Personal information about individuals \&predicts good or bad credit.\\
    \hline
    Bank Marketing	& 16	& Age	& 45211	& Contains marketing data of a Portuguese bank. Goal predicting term deposit.\\
    \hline
    MEP	& 1831	& Race	& 35428	& Surveys of families, individuals, medical providers, employers. Target is “Utilization”.\\
    \hline 
    \end{tabular}
    }
  \label{table 1}%
\end{table*}%


\subsubsection{Optimization Effectiveness Metrics} Although models' performance and fairness can prove the strength of the proposed method, we remain to need a metric to indicate the quantitative effectiveness directly. Thus, we define $ROO_{acc}$ (rate of optimizing accuracy) as following:
\begin{equation}
    ROO_{acc} = \frac{acc_{o} - {acc_{d}}}{acc_{d}} * 100\%
\end{equation}
Where $acc_{o}$ denotes accuracy after optimized, $acc_{d}$ demotes the default accuracy. Similarly, we define $ROO_{MSPD}$, $ROO_{AOD}$, $ROO_{EOD}$, $ROO_{precision}$, $ROO_{recall}$, $ROO_{f1score}$ as well. As for performance-related metrics, the symbols $+(increase)/-(decrease)$ mean increase/decrease performance while for fairness-related metrics the symbols $+(increase)/-(decrease)$ mean increase/decrease unfairness and bias. The values indicate the effectiveness.



\subsection{Research Questions}
\shangwen{Consider introduce this subsection first in this section.}
We evaluate the proposed method via answer the following research questions.
\begin{itemize}[leftmargin = 10 pt]
    \item \textbf{RQ1: To what extent can CUFF achieve a trade-off between effectiveness and fairness? } We answer that CUFF can significantly mitigate datasets and model bias by comparing default models and CUFF models with the fairness and optimization effectiveness metrics. 
\end{itemize}

\begin{itemize}[leftmargin = 10 pt]
    \item \textbf{RQ2: To what extent can multi objective optimization enhance the effectiveness and fairness of CUFF?} We answer that CUFF can optimizes performance and fairness simultaneously by comparing default models and CUFF models with the performance, fairness and optimization effectiveness metrics. 
\end{itemize}

\begin{itemize}[leftmargin = 10 pt]
    \item \textbf{RQ3: Competitiveness in Pre-processing Methods.} What's CUFF's strength compared with the current SOTA pre-processing method? We answer this research question by comparing CUFF with the SOTA pre-processing method Fair-SMOTE \cite{chakraborty2021bias}, Fairway \cite{chakraborty2020fairway} and another approach REW \cite{kamiran2012data}.
\end{itemize}

\begin{itemize}[leftmargin = 10 pt]
    \item \textbf{RQ4: Competitiveness in In-processing Methods and Post-processing.} What's CUFF strength compared with current SOTA in-processing and post-processing methods? We answer this research question by comparing CUFF with the SOTA in-processing method MAAT \cite{chen2022maat} and post-processing method \cite{kamiran2012decision}.
\end{itemize}

\begin{itemize}[leftmargin = 10 pt]
    \item \textbf{RQ5: To what extent can CUFF generalize to different datasets?} This research question is answered by illustrating the effectiveness of experiments in different benchmark datasets and tasks with different algorithms.
\end{itemize}



\begin{abstract}
With the prevalence of data-driven decision-making algorithms, ethical issues such as fairness problems receive considerable attention. Unfair models and machine discrimination exist ubiquitously because machine learning models' effectiveness significantly depends on the data quality, while the datasets are usually biased in the real-world. In some critical decision-making systems, the unfair models might affect the allocation of public social resources, exacerbating discrimination against a particular group and causing social disruption. Unlike the current pre-processing state-of-the-art method sacrificing performance for fairness, we propose CUFF, an explainable bias mitigation strategy via analyzing the causality between features and label. The decision-making tasks are modeled as a Structural Causal Model, and we take causal intervention to calculate the causal effect toward to predicted decision quantitatively. Multiple-Objective Optimization is introduced to process the conflict between performance and fairness for a fairer model. In order comprehensively evaluate CUFF, we conducted our experiments in six tasks on four public benchmark datasets with five typical machine learning algorithms. Compared with the six existing approaches, we realized the state-of-the-art fairness metrics without losing too much performance, even boosting the fairness and performance simultaneously in most tasks.

\end{abstract}

answer rq 1
Table 2-3 shows the compared result of FITNESS and other pre-processing methods, while Table 4 shows the result of FITNESS and in/post-processing methods in various datasets.

        MEP	& 1831	& Race	& 35428	& Surveys of families, individuals, medical providers, employers. Target is “Utilization”.\\
        \hline 
        
        
        
\subsubsection{Optimization Effectiveness Metrics} Although models' performance and fairness can prove the strength of the proposed method, we remain to need a metric to indicate the quantitative effectiveness directly. Thus, we define $OG$ (Optimization Gain) as following:
\begin{equation}
\begin{aligned}
    OG = & (P1_{o}-P1_{d})+(P2_{o}-P2_{d})-(AOD_{o}-AOD_{d})\\&-(EOD_{o}-EOD_{d})
\end{aligned}
\end{equation}
Where $P1_{o}$ denotes optimized accuracy, $P1_{d}$ demotes default accuracy, $P2_{o}$ denotes optimized F1 Score, $P2_{d}$ demotes default F1 Score, $AOD_{o}$ denotes optimized $AOD$, $AOD_{d}$ demotes default $AOD$, $EOD_{o}$ denotes optimized $EOD$, $EOD_{d}$ demotes default $EOD$. A higher OG value is what we expected. \shangwen{Is OG used by previous study? What is its meaning should be introduced more? Also why use AOD and EOD but not SPD?}


Nowadays, recommendation systems are widely-used in web services. Such systems are generally based on machine learning models, whose quality is evidently affected by the dataset quality    \cite{mehrabi2021survey, tsioutsiouliklis2022link, li2021user}. An ideal dataset is expected to be class-balanced, diverse, large-scale, and confound-free. 
However, in practice, the dataset is usually biased and limited in size because of the cost and privacy policy constrain \cite{mehrabi2021survey}. Imbalanced class distribution and confounds decrease the model's performance. At the same time, the bias with respect to the human sensitive features may produce prejudice and discrimination, which are likely to cause severe fairness problems and social disruption to the learned model. 

The interaction between users and web services or applications aggregates the unfairness in data and model preferences as well \cite{mehrabi2021survey}. In such scenarios as social media push and online shopping, users' clicks produce more similar data exaggerating model preferences. Though web service providers and advertisers favor these results, they put the user at a disadvantage, \ie a cocoon filled with homogeneous information, which obviously runs counter to the web spirit of openness, freedom and equality \cite{assembly1948universal, ji2020crack}. Thus,  in Web, AI, ML and SE communities, lots of work aims to address the bias and fairness problems in modern web services.


\subsection{Sensitive Features}
Sensitive features or protected attributes are mentioned and explained in many related works, while they remain lack a clear definition based on objective facts. To avoid misunderstanding, in this paper, a sensitive feature or protected attribute is referred to an individual's innate, lifelong nature (e.g., blood type, gender, race, skin color) related to genes that cannot be modified except for certain diseases or medical treatments.


\noindent $\bullet$ We first introduced the intervention to bias mitigation.

\noindent $\bullet$ We proposed FITNESS which can mitigate data and model bias simultaneously.

\noindent $\bullet$ We proposed FITNESS which can enhance model fairness and performance simultaneously.

\noindent $\bullet$ We conducted large-scale experiments and opened all the data and codes to the public to help others reproduce or extend the research.

==> Z_draft_result.tex <==


\subsection{Research Questions}
\shangwen{Consider introduce this subsection first in this section.}
We evaluate the proposed method via answer the following research questions.
\begin{itemize}[leftmargin = 10 pt]
    \item \textbf{RQ1: How About the Multi-Objective Optimization Effectiveness of FITNESS?} To answer this research question, we compared FITNESS models with default models in 4 performance metrics and two fairness metrics. 
\end{itemize}

\begin{itemize}[leftmargin = 10 pt]
    \item \textbf{RQ2: Is FITNESS More Competitive Than Existing Pre-processing Methods?}
    We answer this RQ by comparing FITNESS with existing state-of-the-art pre-processing methods Fair SMOTE \cite{chakraborty2021bias}, Fairway\cite{chakraborty2020fairway} and REW \cite{kamiran2012data}. To alleviate confounding, we designed controlled variable experiments that compare each method in the same dataset, different ML algorithms and the same ML algorithms, different datasets separately.
\end{itemize}

\begin{itemize}[leftmargin = 10 pt]
    \item \textbf{RQ3: Is FITNESS More Competitive Than Existing In/post-processing Methods?} 
    Similar to RQ 2, we answer this RQ via comparing FINTSEE with state-of-the-art in-processing method and post-processing method MAAT \cite{chen2022maat} , ADV \cite{zhang2018mitigating} and ROC \cite{kamiran2012decision}.
\end{itemize}

\begin{itemize}[leftmargin = 10 pt]
    \item \textbf{RQ4: How about the FITNESS applicability?} 
    This research question is answered by illustrating the effectiveness of experiments in different benchmark datasets and tasks with varying algorithms of ML. 
\end{itemize}

\subsection{Experiment Design}
Here we introduce the experiment design in detail to help other researchers reproduce our method easily. To comprehensively evaluate the approach, we select four public benchmark datasets and five typical machine learning algorithms, including Logistical Regression (LR) , Support Vector Machine (SVM), Naive Bayes (NB), Random Forest (RF) and Decision Tree (DT) \cite{chen2022maat, chakraborty2021bias}. Besides, to avoid confounding, we use the machine learning algorithms integrated in the Scikit-Learn library \cite{scikit-learn, sklearn_api} and Optimization algorithms in the Scikit-opt library c\cite{misc_Scikit-opt}. Every experiment repeats fifty times and selects the mean. 

%result
In this section, we present our experiments result by answering the proposed research question. Because of the tremendous number of experiments, to comprehensively compare each method, we have to use tables instead of intuitive and vivid graphs to present the result. To enhance the legibility, we mark the cells with three colors. Darker indicates the top level; lighter indicates the medium level and white indicates the worse level. All the result is the average of 50 times run. "default" means the unmitigated model.
\subsection{RQ1: How About the Multi-Objective Optimization Effectiveness?}

We evaluate the MOO effectiveness via the comparison of default models and FITNESS-mitigated models. Table 2 shows the result of Logistic Regression (LR) in different datasets and tasks, while Table 3 shows the result of different machine learning algorithms in the Adult dataset. Compared with the default models, all FITNESS-mitigated models obtained significant improvement in both performance and fairness. In the experiments of varying datasets with the LR algorithm, the recall increased by 36.69\%, precision increased by 14.54\%, accuracy increased by 5.62\%, F1 Score increased by 24.16\%, AOD decreased by41.83\% and EOD decreased by 68.36\%. In the experiments of varying algorithms in the Adult dataset, the recall increased by 99.03\%, precision increased by 12.66\%, accuracy increased by 0.41\%, F1 Score increased by 54.54\%, AOD decreased by 64.07\% and EOD decreased by 83.82\%. Hence, we think FITNESS realized excellent bias mitigation and trade-off for model fairness and performance. 

~\

\noindent \textbf{The bias mitigation and MOO effectiveness of FITNESS is satisfactory.}
~\
\subsection{RQ2: Is FITNESS More Competitive than Existing Pre-processing Methods?}
From Table 2 and Table 3, we can see that almost all FITNESS models are marked by a "top-level" color block. As well we can see the state-of-the-art method Fair-SMOTE models realized excellent fairness. However, their performance metrics had a significant drop. Most of them are marked by "worse level". The recall decreased by XX, precision decreased by XX, accuracy decreased by XX and F1 Score decreased by XX on average. To better evaluate the effectiveness of each mitigation method, we define a metric Optimization Gain (OG) by two performance metrics and two fairness metrics in Section 4. Through calculation, FITNESS obtained the highest OG value among all the pre-processing methods. The OG of FITNESS' is XX higher than REW's, XX higher than Fairway' and XX higher than Fair SMOTE's. Hence, we answer research question 2:

~\

\textbf{FITNESS is Evidently More Competitive than Existing Pre-processing Methods.}
~\

\subsection{RQ3: Is FITNESS More Competitive than Existing In/post-processing Methods?} 
In-processing and post-processing methods are model bias mitigating strategies instead of data mitigation approaches. Thus, we compared them with FITNESS separately.  Almost all the FITNESS models are marked by top-level color blocks. Specifically, in recall metric, FITNESS models lost by XX on average while the precision increased by XX, accuracy increased by XX and F1 Score increased by XX. Furthermore, FITNESS increased AOD by XX and EOD by XX.
On the contrary, rare other methods' models are marked by top-level color blocks. ROC realized good fairness metrics in LR and SVM experiments but failed in RF. MAAT successfully decreased the EOD value while it increased the AOD. As for the OG, FITNESS held the highest value, XX higher than ADV, XX higher than AOC and XX higher than MAAT. Only FITNESS showed stability and effectiveness in mitigating bias and obtaining fair models among the four mitigation methods. For answering research question 3, that is no doubt that:

~\

\textbf{FITNESS is Overwhelming Competitive than Existing In-processing and Post-processing Methods.}
~\


\subsection{RQ4: Applicability.}
We conducted the experiments in thirty different combinations of dataset, task and algorithm.


Among all the experiments (6*5*50=1500), the 99.5\% FITNESS model performs better than the default model without any negative effect. Hence, we are confident that FITNESS can be generalized to other datasets and other machine learning algorithms.


\subsection{Why FITNESS?}
At least three strengths support the view that FITNESS is an excellent bias mitigation method.

\textbf{Uncompromising:}
Among all the experiments we conducted, FITNESS 100\% enhanced the model fairness by 89\% on average while only 3\% model decreased performance by 1\%. In a nutshell, compared with existing approaches, FITNESS realized the best fairness and performance trade-off. Furthermore, we can confidently rebut Berk \cite{berk2021fairness} that it is possible to achieve fairness and high performance simultaneously in universal cases.

\textbf{Versatility and Applicability:} As a pre-processing method, FITNESS is more applicable and versatile, as it mitigates bias through processing data. Hence, FITNESS performs similarly in various machine learning algorithms without too much effectiveness fluctuating. Furthermore, FITNESS can train discrimination-free models independently and work as a data mitigation tool to combine with other in/post-processing methods for higher optimization gain.


\textbf{Explainability:} FITNESS is the first bias mitigation method providing causal explainability. Most previous pre-processing methods are trapped in the scope of balancing bata with oversampling, under-sampling and synthesizing new data samples. They didn't think further about why balancing methods work while FITNESS calculates quantitative causal effect between sensitive feature and label and interdict the unreliable correlation.


\subsection{Threats to Validity}
From a causality perspective, machine learning software has two kinds of fairness problems. One is that the sensitive features which need to be protected are causal-free with the label. Another is that the sensitive features are causally related to the label. The causal de-correlated-based FITNESS is applicable for both two problems. The only difference is that FITNESS would not decrease any performance in the first kind; FITNESS needs to sacrifice a small part of the performance as the cost for fairness in the second kind.

\subsection{Potential Opportunities}
Although this paper focuses on the fairness problem, we obtained an extra benefit from FITNESS. After causal de-correlation, the learned model performs more robust and stable in Out-of-Distribution (OOD) scenarios. It will be a direction guiding our further study.


==> Z_draft_result_2.tex <==
\subsection{Comparison with Pre-processing Methods}
\subsubsection{\textbf{Results of Setup 1}}

According to Table \ref{tab:exp1}, we observe that most of the FITNESS models are located in the top-level domain. Only three metrics are out of top-level such as recall in the German-Sex task, but they actually are very close to the top values.
Compared with the default models, FITNESS models perform better in fairness metrics.
For instance, the ADO decreases by 41.82\%  and EOD decreases by 68.36\%, on average. As for the model performance, the FITNESS model decreases a little bit with respect to precision and accuracy in the German-Sex task, while all the performance metrics experience a significant improvement in the rest tasks. These results show that FITNESS can mitigate data bias, and enhance model performance and fairness simultaneously.

When it comes to the other pre-processing methods, we observe that most of them can actually alleviate the unfairness problem. However, these methods can not optimize the performance like FITNESS. 
For instance, Fairway experienced the degradation of the model performance in most tasks, especially in the Adult-Sex task where its recall drops by 40.47\% and the F1 Score drops by 22.22\%. REW performed well in accuracy metrics in the Adult-Race and Adult-Sex tasks but did not perform as well as FITNESS in reducing unfairness metrics. Compared with the existing pre-processing mitigation strategies, FITNESS can dominate other methods because FITNESS is the only bias mitigation technique that can realize excellent trade-offs between performance and fairness in different datasets.

\subsubsection{\textbf{Results of Setup 2}}
Similar to Experiment 1, all FITNESS models are located in the top-level domain. From a bias mitigation perspective, Fair SMOTE obtained minimum AOD and EOD metrics while FITNESS performed distinguished as well, and the fairness metrics were very close to those from Fair SMOTE. However, regarding the performance, FITNESS obtained almost all the highest performance except precision in the RF group and accuracy in the LR group. 
Significantly, FITNESS boosted models' recall by 99.03\% and the F1 Score by 54.54\% on average. Besides, in the same task, FITNESS showed similar performance optimization and bias mitigation effectiveness among diverse machine learning algorithms. Hence, from this comparison, we conclude that FITNESS outperforms all existing pre-processing methods on the trade-off between fairness and performance.

\subsubsection{\textbf{Reason Analysis}}
According to the result, we conduct reason analysis on: (1) enhancing fairness and performance simultaneously; (2) stability in varying algorithms; (3) stability in varying datasets.

\textbf{(1) Enhancing fairness and performance simultaneously. }
Although four pre-processing methods showed significant data bias mitigation effectiveness, they have varying impacts on the performance because of the different core ideas of these methods.
Reweighing (REW) alleviates data bias via setting different weights to features \cite{kamiran2012data}. This method cannot handle the impact on model performance, and it is difficult to determine the optimal weight for each feature in varying datasets, which causes the effectiveness to fluctuate. For example, the bias mitigation effect of REW is not evident in the Adult-Sex task with SVM. REW cannot significantly enhance model performance as well. 
The behind intuitions of Fairway and Fair SMOTE are similar. Both of the two methods mitigate bias by removing ambiguous data points \cite{chakraborty2020fairway, chakraborty2021bias}. This radical and high-risk strategy might cause the model to be under-fitting because of removing too many data points. The results in Table \ref{tab:exp1} and Table \ref{tab:exp2} verified our concern that in almost all the experiments, Fairway caused varying degrees of decreases of the model performance. Fair SMOTE performed slightly better than Fairway as it mutated new data points to compensate for the removed data. However, the mutation effect is limited as well because Fair SMOTE significantly decreased model performance in the Adult dataset.
With regard to FITNESS, causal de-correlation did not remove any data, which keeps the potential of enhancing modal performance. The objective function of MOO includes two fairness metrics and two performance metrics. It enables FITNESS to boost model performance and fairness simultaneously. These two designs make FITNESS outperform all existing pre-processing methods.

\textbf{(2) Stability in varying algorithms.}
The pre-processing method trains fair models via mitigating dataset bias, which avoids performing any customized optimization or modification to the algorithms. Hence, different algorithms would not directly affect the modal's effectiveness after the mitigation of the unfairness, which is supported by the stable and excellent effectiveness of FITNESS in experiments of varying algorithms.
However, the experiments on Fairway presented contrary facts. Compared with the default model, Fairway successfully mitigated model bias and improved the model recall in RF and SVM but decreased the model recall score by 40.47\% in the LR experiment. We suppose the algorithms' sensitivity to data causes the gap because Fairway is an aggressive technique mitigating bias via removing ambiguous data points. This method might shift data distribution in the dataset, which led to the significant differences among the algorithms' performance. 
Also, Fair SMOTE ameliorated this problem by generating new data points and kept stable effectiveness in various machine learning algorithms. 
REW showed stability as well because it kept the original data, though the effectiveness is not very distinguished. 
As for FITNESS, de-correlation did not delete any data points, which guarantees the datasets' integrity, while the adopted MOO help the model reach a high degree of effectiveness.
% In such datasets, MOO can keep high .

\textbf{(3) Stability in varying datasets.}
Similar to the stability in varying algorithms, the two methods that did not remove data points (\ie FITNESS and REW), performed stably in various datasets and tasks.
The difference is that FITNESS keeps the highest effectiveness while REW keeps a medium level of effectiveness. For the same reason as the above analysis, Fairway performed varying in different datasets and tasks. However, what should be noticed is that Fair SMOTE performed stably in varying algorithms but fluctuated in varying datasets. In the Adult and Compas datasets, Fair SMOTE decreased model performance, though it kept high effectiveness in mitigating bias. This phenomenon implies that mutating high-quality data points is extremely challenging.


\subsection{Comparison with In/Post-processing Methods}
\subsubsection{\textbf{Results of Setup 3}}
Table \ref{tab:exp3} presented the comparison results among FITNESS and state-of-the-art in-processing method MAAT \cite{chen2022maat}, Adversarial Debiasing (ADV) \cite{zhang2018mitigating} and post-processing method Reject Option Based Classification (ROC) \cite{kamiran2012decision}. It is clear that all FITNESS models are located in the top-level domain. Moreover, all fairness metrics of FITNESS are best. About other methods, ROC performed distinguished with LR and SVM. MAAT showed slight bias mitigation effectiveness, while ADV magnified model bias. As for performance, compared with the default model, all mitigation methods decreased a little recall score, but FITNESS was still better than others. In the rest performance metrics, ADV, ROC and MAAT did not affect the model much, while FITNESS evidently improved the precision and accuracy. Thus we can confidently declare that FITNESS outperforms all existing in-processing and post-processing methods.

\subsubsection{\textbf{Reason Analysis}}
We recall that we have already analyzed why FITNESS can stably handle model performance and fairness in varying scenarios.
% FITNESS has already been analyzed why it can stably handle model performance and fairness in varying scenarios. 
In this part, we focused on analyzing other methods from the same perspective as pre-processing methods. The results showed none of them can optimize performance when enhancing fairness. These approaches did not break the original datasets, which enabled them to realize the same stable performance as the default model with different algorithms. Nonetheless, as for fairness metrics, these approaches had rather different performance. 

\textbf{(1) MAAT.} MAAT kept stable but had slight effectiveness in mitigating model bias. Its core idea is to train the fairness and performance models separately and combines them with different weights for the final decision. This method is more like a “zero-sum game”. If MAAT wants to enhance model fairness, it must set a high weight to the fairness model which might damage performance and vice versa. The best result of this method is keeping the performance when increasing fairness, as shown in Table \ref{tab:exp3}, instead of boosting both of them.

\textbf{(2) ROC.} 
If a prediction is near the threshold and the model assigns a favorable label to the privileged group or assigns an unfavorable label to the unprivileged group, ROC will reverse the prediction to reduce the model bias. This method relays on a hypothesis that most bias and discrimination occur near the threshold, which still needs to be verified. The result in RF showed the method is not always effective.


\textbf{(3) ADV.}
ADV is a method based on adversarial learning that hides the sensitive feature in the training procession and predicts the feature as well as the label. In a biased dataset, if the feature was predicted correctly, the model would be punished and vice versa if the feature was incorrectly predicted. This method is more likely to make the privileged group in the dataset become the unprivileged, instead of treating them equally. The results in Table \ref{tab:exp3} showed ADV magnified model bias.











==> exp1.tex <==
%\subsection{Effectiveness of \toolname}
%\label{subsec:rq1}


% Table generated by Excel2LaTeX from sheet 'Sheet2'
% Table generated by Excel2LaTeX from sheet 'Sheet2'
% Table generated by Excel2LaTeX from sheet 'Sheet2'
% Table generated by Excel2LaTeX from sheet 'T1'
% Table generated by Excel2LaTeX from sheet 'T1'
% Table generated by Excel2LaTeX from sheet 'T1'
\begin{table}[htbp]
  \centering
  \caption{The results of Setup 1. "Default" means unmitigated bias; "Compas-Sex" means "in Compas dataset, mitigate sex bias"; "R" means Recall; "P" means Precision; "Acc" means accuracy; "F1" means F1 Score. "(M)SPD" means in FITNESS, the cell is "MSPD" and in other cases, the cell is "SPD". As for Recall, Precision, Accuracy and F1 Score, the higher, the better. As for AOD, EOD, (M)SPD, the lower, better. the \colorbox[rgb]{ .22,  .525,  .8}{darkest} cells means the top rank,
the \colorbox[rgb]{ .475,  .678,  .867}{lighter} cells and the \colorbox[rgb]{ .867,  .922,  .969}{lightest} indicate rank two and rank three, respectively; and the white cells means last rank.  The value in each cell indicates the mean value of 50 runs. The same as Table \ref{tab:exp2} and \ref{tab:exp3}.
}
  \vspace{-2ex}
\resizebox{\columnwidth}{!}{
     \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
   \Xhline{1.1pt}
    \rowcolor[rgb]{ .682,  .667,  .667} \textbf{Task} & \textbf{Method} & \textbf{R} & \textbf{P} & \textbf{Acc} & \textbf{F1} & \textbf{AOD} & \textbf{EOD} & \textbf{(M)SPD} \bigstrut\\
   \Xhline{1.1pt}
    \multirow{5}[10]{*}{\begin{turn}{90}Compas-Sex\end{turn}} & Default & \cellcolor[rgb]{ .475,  .678,  .867}0.73  & \cellcolor[rgb]{ .867,  .922,  .969}0.66  & 0.64  & 0.61  & \cellcolor[rgb]{ .475,  .678,  .867}0.05  & 0.14  & 0.18  \bigstrut\\
\cline{2-9}          & REW   & \cellcolor[rgb]{ .867,  .922,  .969}0.65  & \cellcolor[rgb]{ .867,  .922,  .969}0.66  & \cellcolor[rgb]{ .867,  .922,  .969}0.66  & \cellcolor[rgb]{ .867,  .922,  .969}0.65  & \cellcolor[rgb]{ .475,  .678,  .867}0.04  & \cellcolor[rgb]{ .475,  .678,  .867}0.02  & 0.04  \bigstrut\\
\cline{2-9}          & Fairway & 0.56  & 0.57  & 0.58  & 0.58  & \cellcolor[rgb]{ .475,  .678,  .867}0.03  & \cellcolor[rgb]{ .475,  .678,  .867}0.03  & 0.06  \bigstrut\\
\cline{2-9}          & Fair SMOTE & 0.62  & 0.56  & 0.55  & 0.65  & \cellcolor[rgb]{ .475,  .678,  .867}0.02  & \cellcolor[rgb]{ .475,  .678,  .867}0.05  & 0.08  \bigstrut\\
\cline{2-9}          & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.72  & \cellcolor[rgb]{ .22,  .525,  .8}0.81  & \cellcolor[rgb]{ .475,  .678,  .867}0.72  & \cellcolor[rgb]{ .475,  .678,  .867}0.72  & \cellcolor[rgb]{ .475,  .678,  .867}0.03  & \cellcolor[rgb]{ .475,  .678,  .867}0.03  & 0.04  \bigstrut\\
     \Xhline{1.1pt}
    \multirow{5}[10]{*}{\begin{turn}{90}Compas-Race\end{turn}} & Default & \cellcolor[rgb]{ .867,  .922,  .969}0.69  & \cellcolor[rgb]{ .867,  .922,  .969}0.65  & 0.64  & \cellcolor[rgb]{ .867,  .922,  .969}0.68  & \cellcolor[rgb]{ .475,  .678,  .867}0.05  & 0.11  & 0.12  \bigstrut\\
\cline{2-9}          & REW   & \cellcolor[rgb]{ .867,  .922,  .969}0.65  & \cellcolor[rgb]{ .867,  .922,  .969}0.66  & \cellcolor[rgb]{ .867,  .922,  .969}0.66  & \cellcolor[rgb]{ .867,  .922,  .969}0.65  & \cellcolor[rgb]{ .475,  .678,  .867}0.03  & \cellcolor[rgb]{ .475,  .678,  .867}0.04  & 0.02  \bigstrut\\
\cline{2-9}          & Fairway & \cellcolor[rgb]{ .867,  .922,  .969}0.65  & \cellcolor[rgb]{ .867,  .922,  .969}0.66  & \cellcolor[rgb]{ .867,  .922,  .969}0.66  & \cellcolor[rgb]{ .867,  .922,  .969}0.65  & 0.12  & 0.07  & 0.14  \bigstrut\\
\cline{2-9}          & Fair SMOTE & 0.62  & 0.56  & 0.55  & 0.66  & \cellcolor[rgb]{ .475,  .678,  .867}0.01  & \cellcolor[rgb]{ .475,  .678,  .867}0.05  & 0.06  \bigstrut\\
\cline{2-9}          & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.71  & \cellcolor[rgb]{ .475,  .678,  .867}0.73  & \cellcolor[rgb]{ .475,  .678,  .867}0.71  & \cellcolor[rgb]{ .475,  .678,  .867}0.71  & 0.06  & \cellcolor[rgb]{ .475,  .678,  .867}0.05  & 0.09  \bigstrut\\
    \Xhline{1.1pt}
    \multirow{5}[10]{*}{\begin{turn}{90}Adult-Sex\end{turn}} & Default & 0.42  & 0.69  & \cellcolor[rgb]{ .475,  .678,  .867}0.83  & 0.54  & 0.12  & 0.24  & 0.21  \bigstrut\\
\cline{2-9}          & REW   & 0.74  & \cellcolor[rgb]{ .867,  .922,  .969}0.79  & \cellcolor[rgb]{ .475,  .678,  .867}0.83  & \cellcolor[rgb]{ .867,  .922,  .969}0.76  & 0.08  & 0.15  & 0.08  \bigstrut\\
\cline{2-9}          & Fairway & 0.25  & 0.70  & 0.72  & 0.42  & \cellcolor[rgb]{ .475,  .678,  .867}0.02  & \cellcolor[rgb]{ .475,  .678,  .867}0.03  & 0.01  \bigstrut\\
\cline{2-9}          & Fair SMOTE & 0.71  & 0.25  & 0.51  & 0.73  & \cellcolor[rgb]{ .475,  .678,  .867}0.01  & \cellcolor[rgb]{ .475,  .678,  .867}0.02  & 0.02  \bigstrut\\
\cline{2-9}          & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.82  & \cellcolor[rgb]{ .475,  .678,  .867}0.82  & \cellcolor[rgb]{ .475,  .678,  .867}0.82  & \cellcolor[rgb]{ .475,  .678,  .867}0.82  & \cellcolor[rgb]{ .475,  .678,  .867}0.04  & \cellcolor[rgb]{ .475,  .678,  .867}0.03  & 0.01  \bigstrut\\
 \Xhline{1.1pt}
    \multirow{5}[10]{*}{\begin{turn}{90}Adult-Race\end{turn}} & Default & 0.42  & 0.69  & \cellcolor[rgb]{ .475,  .678,  .867}0.81  & 0.52  & 0.06  & 0.15  & 0.16  \bigstrut\\
\cline{2-9}          & REW   & \cellcolor[rgb]{ .867,  .922,  .969}0.75  & \cellcolor[rgb]{ .475,  .678,  .867}0.80  & \cellcolor[rgb]{ .475,  .678,  .867}0.84  & \cellcolor[rgb]{ .867,  .922,  .969}0.77  & \cellcolor[rgb]{ .475,  .678,  .867}0.03  & 0.06  & 0.04  \bigstrut\\
\cline{2-9}          & Fairway & \cellcolor[rgb]{ .867,  .922,  .969}0.76  & \cellcolor[rgb]{ .475,  .678,  .867}0.80  & \cellcolor[rgb]{ .475,  .678,  .867}0.84  & \cellcolor[rgb]{ .867,  .922,  .969}0.78  & \cellcolor[rgb]{ .475,  .678,  .867}0.05  & 0.07  & 0.09  \bigstrut\\
\cline{2-9}          & Fair SMOTE & 0.70  & 0.51  & 0.72  & 0.62  & \cellcolor[rgb]{ .475,  .678,  .867}0.04  & \cellcolor[rgb]{ .475,  .678,  .867}0.03  & 0.05  \bigstrut\\
\cline{2-9}          & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.82  & \cellcolor[rgb]{ .475,  .678,  .867}0.83  & \cellcolor[rgb]{ .475,  .678,  .867}0.82  & \cellcolor[rgb]{ .475,  .678,  .867}0.82  & \cellcolor[rgb]{ .475,  .678,  .867}0.03  & \cellcolor[rgb]{ .475,  .678,  .867}0.04  & 0.02  \bigstrut\\
  \Xhline{1.1pt}
    \multirow{5}[10]{*}{\begin{turn}{90}Bank-Age\end{turn}} & Default & 0.73  & 0.76  & 0.77  & 0.77  & 0.14  & 0.22  & 0.24  \bigstrut\\
\cline{2-9}          & REW   & 0.68  & 0.79  & \cellcolor[rgb]{ .475,  .678,  .867}0.89  & 0.71  & \cellcolor[rgb]{ .475,  .678,  .867}0.03  & 0.06  & 0.02  \bigstrut\\
\cline{2-9}          & Fairway & 0.71  & 0.73  & 0.71  & 0.73  & \cellcolor[rgb]{ .475,  .678,  .867}0.04  & \cellcolor[rgb]{ .475,  .678,  .867}0.03  & 0.03  \bigstrut\\
\cline{2-9}          & Fair SMOTE & 0.76  & 0.72  & 0.72  & 0.74  & \cellcolor[rgb]{ .475,  .678,  .867}0.05  & 0.07  & 0.03  \bigstrut\\
\cline{2-9}          & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.88  & \cellcolor[rgb]{ .475,  .678,  .867}0.87  & \cellcolor[rgb]{ .475,  .678,  .867}0.88  & \cellcolor[rgb]{ .475,  .678,  .867}0.87  & \cellcolor[rgb]{ .475,  .678,  .867}0.05  & 0.09  & 0.07  \bigstrut\\
    \Xhline{1.1pt}
 
    \multirow{5}[10]{*}{\begin{turn}{90}German-Sex\end{turn}} & Default & \cellcolor[rgb]{ .867,  .922,  .969}0.66  & \cellcolor[rgb]{ .22,  .525,  .8}0.70  & \cellcolor[rgb]{ .22,  .525,  .8}0.74  & \cellcolor[rgb]{ .475,  .678,  .867}0.67  & 0.10  & 0.07  & 0.11  \bigstrut\\
\cline{2-9}          & REW   & \cellcolor[rgb]{ .867,  .922,  .969}0.66  & \cellcolor[rgb]{ .867,  .922,  .969}0.69  & \cellcolor[rgb]{ .22,  .525,  .8}0.74  & \cellcolor[rgb]{ .475,  .678,  .867}0.67  & \cellcolor[rgb]{ .333,  .592,  .827}0.05  & \cellcolor[rgb]{ .333,  .592,  .827}0.03  & 0.05  \bigstrut\\
\cline{2-9}          & Fairway & \cellcolor[rgb]{ .867,  .922,  .969}0.67  & \cellcolor[rgb]{ .867,  .922,  .969}0.69  & \cellcolor[rgb]{ .22,  .525,  .8}0.74  & \cellcolor[rgb]{ .475,  .678,  .867}0.67  & 0.06  & \cellcolor[rgb]{ .333,  .592,  .827}0.03  & 0.05  \bigstrut\\
\cline{2-9}          & Fair SMOTE & 0.62  & \cellcolor[rgb]{ .22,  .525,  .8}0.71  & 0.64  & \cellcolor[rgb]{ .22,  .525,  .8}0.71  & \cellcolor[rgb]{ .333,  .592,  .827}0.05  & \cellcolor[rgb]{ .333,  .592,  .827}0.05  & 0.05  \bigstrut\\
\cline{2-9}          & FITNESS & \cellcolor[rgb]{ .22,  .525,  .8}0.71  & \cellcolor[rgb]{ .333,  .592,  .827}0.69  & \cellcolor[rgb]{ .22,  .525,  .8}0.71  & \cellcolor[rgb]{ .475,  .678,  .867}0.67  & \cellcolor[rgb]{ .333,  .592,  .827}0.05  & \cellcolor[rgb]{ .333,  .592,  .827}0.03  & 0.07  \bigstrut\\
    \hline
    \Xhline{1.1pt}
    \end{tabular}%
    }
  \label{tab:exp1}%
\end{table}%



 


   

==> exp2.tex <==
%\subsection{The Impact of Input Quality on \toolname}
%\label{subsec:rq2}
% Table generated by Excel2LaTeX from sheet 'Sheet2'
% Table generated by Excel2LaTeX from sheet 'Sheet3'
% Table generated by Excel2LaTeX from sheet 'Sheet4'
% Table generated by Excel2LaTeX from sheet 'Table-3-in-post-processing'
% Table generated by Excel2LaTeX from sheet 'T3'
% Table generated by Excel2LaTeX from sheet 'Sheet7'
% Table generated by Excel2LaTeX from sheet 'T2'

\begin{comment}


\begin{table}[htbp]
  \centering
  \caption{The results of Setup 2. "Alg." means "algorithm".}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \Xhline{1.1pt}
    \rowcolor[rgb]{ .682,  .667,  .667} \textbf{Task} & \textbf{Alg.} & \textbf{Method} & \textbf{R} & \textbf{P} & \textbf{Acc} & \textbf{F1} & \textbf{AOD} & \textbf{EOD} & \textbf{(M)SPD} \bigstrut\\
   \Xhline{1.1pt}
    \multirow{5}[10]{*}{\begin{turn}{-90}Adult-Sex\end{turn}} & \multirow{5}[10]{*}{LR} & Default & 0.42  & 0.69  & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & 0.54  & 0.12  & 0.24  & 0.21 \bigstrut\\
\cline{3-10}          &       & REW   & 0.74  & \cellcolor[rgb]{ .867,  .922,  .969}0.79 & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & \cellcolor[rgb]{ .867,  .922,  .969}0.76 & 0.08  & 0.15  & 0.08 \bigstrut\\
\cline{3-10}          &       & Fairway & 0.25  & 0.7   & 0.72  & 0.42  & \cellcolor[rgb]{ .475,  .678,  .867}0.02 & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & 0.01 \bigstrut\\
\cline{3-10}          &       & Fair SMOTE & 0.71  & 0.51  & 0.73  & 0.62  & \cellcolor[rgb]{ .475,  .678,  .867}0.01 & \cellcolor[rgb]{ .475,  .678,  .867}0.02 & 0.03 \bigstrut\\
\cline{3-10}          &       & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.82 & \cellcolor[rgb]{ .475,  .678,  .867}0.82 & \cellcolor[rgb]{ .475,  .678,  .867}0.82 & \cellcolor[rgb]{ .475,  .678,  .867}0.82 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & 0.01 \bigstrut\\
    \hline
    \multirow{5}[10]{*}{\begin{turn}{-90}Adult-Sex\end{turn}} & \multirow{5}[10]{*}{RF} & Default & 0.51  & 0.72  & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & 0.59  & 0.09  & 0.17  & 0.17 \bigstrut\\
\cline{3-10}          &       & REW   & \cellcolor[rgb]{ .867,  .922,  .969}0.76 & \cellcolor[rgb]{ .867,  .922,  .969}0.79 & \cellcolor[rgb]{ .475,  .678,  .867}0.84 & \cellcolor[rgb]{ .867,  .922,  .969}0.77 & 0.07  & 0.06  & 0.18 \bigstrut\\
\cline{3-10}          &       & Fairway & 0.68  & \cellcolor[rgb]{ .475,  .678,  .867}0.85 & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & 0.71  & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & 0.09 \bigstrut\\
\cline{3-10}          &       & Fair SMOTE & 0.69  & 0.53  & 0.78  & 0.6   & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & 0.1 \bigstrut\\
\cline{3-10}          &       & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.84 & \cellcolor[rgb]{ .475,  .678,  .867}0.84 & \cellcolor[rgb]{ .475,  .678,  .867}0.84 & \cellcolor[rgb]{ .475,  .678,  .867}0.84 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & 0.02 \bigstrut\\
    \hline
    \multirow{5}[10]{*}{\begin{turn}{-90}Adult-Sex\end{turn}} & \multirow{5}[10]{*}{SVM} & Default & 0.35  & \cellcolor[rgb]{ .475,  .678,  .867}0.81 & \cellcolor[rgb]{ .475,  .678,  .867}0.82 & 0.49  & 0.1   & 0.24  & 0.14 \bigstrut\\
\cline{3-10}          &       & REW   & 0.73  & \cellcolor[rgb]{ .475,  .678,  .867}0.8 & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & \cellcolor[rgb]{ .867,  .922,  .969}0.76 & 0.09  & 0.18  & 0.07 \bigstrut\\
\cline{3-10}          &       & Fairway & 0.72  & \cellcolor[rgb]{ .867,  .922,  .969}0.77 & \cellcolor[rgb]{ .475,  .678,  .867}0.8 & 0.71  & 0.11  & 0.12  & 0.17 \bigstrut\\
\cline{3-10}          &       & Fair SMOTE & 0.73  & 0.51  & \cellcolor[rgb]{ .867,  .922,  .969}0.76 & 0.6   & \cellcolor[rgb]{ .475,  .678,  .867}0.02 & \cellcolor[rgb]{ .475,  .678,  .867}0.02 & 0.08 \bigstrut\\
\cline{3-10}          &       & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & 0.02 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:exp2}%
\end{table}%
\end{comment}



% Table generated by Excel2LaTeX from sheet 'T2'
\begin{table}[htbp]
  \centering
  \caption{The results of Setup 2. "Alg." means "algorithm".}
  \vspace{-2ex}
\resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
     \Xhline{1.1pt}
    \rowcolor[rgb]{ .682,  .667,  .667} \textbf{Task} & \textbf{Alg.} & \textbf{Method} & \textbf{R} & \textbf{P} & \textbf{Acc} & \textbf{F1} & \textbf{AOD} & \textbf{EOD} & \textbf{(M)SPD} \bigstrut[t]\\
     \Xhline{1.1pt}
    \multirow{15}[29]{*}{\begin{turn}{90}Adult-Sex\end{turn}} & \multirow{5}[9]{*}{LR} & Default & 0.42  & 0.69  & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & 0.54  & 0.12  & 0.24  & 0.21 \bigstrut[b]\\
\cline{3-10}          &       & REW   & 0.74  & \cellcolor[rgb]{ .867,  .922,  .969}0.79 & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & \cellcolor[rgb]{ .867,  .922,  .969}0.76 & 0.08  & 0.15  & 0.08 \bigstrut\\
\cline{3-10}          &       & Fairway & 0.25  & 0.7   & 0.72  & 0.42  & \cellcolor[rgb]{ .475,  .678,  .867}0.02 & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & 0.01 \bigstrut\\
\cline{3-10}          &       & Fair SMOTE & 0.71  & 0.51  & 0.73  & 0.62  & \cellcolor[rgb]{ .475,  .678,  .867}0.01 & \cellcolor[rgb]{ .475,  .678,  .867}0.02 & 0.03 \bigstrut\\
\cline{3-10}          &       & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.82 & \cellcolor[rgb]{ .475,  .678,  .867}0.82 & \cellcolor[rgb]{ .475,  .678,  .867}0.82 & \cellcolor[rgb]{ .475,  .678,  .867}0.82 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & 0.01 \bigstrut\\
\Xcline{2-10}{1.1pt}          & \multirow{5}[10]{*}{RF} & Default & 0.51  & 0.72  & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & 0.59  & 0.09  & 0.17  & 0.17 \bigstrut\\
\cline{3-10}          &       & REW   & \cellcolor[rgb]{ .867,  .922,  .969}0.76 & \cellcolor[rgb]{ .867,  .922,  .969}0.79 & \cellcolor[rgb]{ .475,  .678,  .867}0.84 & \cellcolor[rgb]{ .867,  .922,  .969}0.77 & 0.07  & 0.06  & 0.18 \bigstrut\\
\cline{3-10}          &       & Fairway & 0.68  & \cellcolor[rgb]{ .475,  .678,  .867}0.85 & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & 0.71  & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & 0.09 \bigstrut\\
\cline{3-10}          &       & Fair SMOTE & 0.69  & 0.53  & 0.78  & 0.6   & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & 0.1 \bigstrut\\
\cline{3-10}          &       & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.84 & \cellcolor[rgb]{ .475,  .678,  .867}0.84 & \cellcolor[rgb]{ .475,  .678,  .867}0.84 & \cellcolor[rgb]{ .475,  .678,  .867}0.84 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & 0.02 \bigstrut\\
\Xcline{2-10}{1.1pt}          & \multirow{5}[10]{*}{SVM} & Default & 0.35  & \cellcolor[rgb]{ .475,  .678,  .867}0.81 & \cellcolor[rgb]{ .475,  .678,  .867}0.82 & 0.49  & 0.1   & 0.24  & 0.14 \bigstrut\\
\cline{3-10}          &       & REW   & 0.73  & \cellcolor[rgb]{ .475,  .678,  .867}0.8 & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & \cellcolor[rgb]{ .867,  .922,  .969}0.76 & 0.09  & 0.18  & 0.07 \bigstrut\\
\cline{3-10}          &       & Fairway & 0.72  & \cellcolor[rgb]{ .867,  .922,  .969}0.77 & \cellcolor[rgb]{ .475,  .678,  .867}0.8 & 0.71  & 0.11  & 0.12  & 0.17 \bigstrut\\
\cline{3-10}          &       & Fair SMOTE & 0.73  & 0.51  & \cellcolor[rgb]{ .867,  .922,  .969}0.76 & 0.6   & \cellcolor[rgb]{ .475,  .678,  .867}0.02 & \cellcolor[rgb]{ .475,  .678,  .867}0.02 & 0.08 \bigstrut\\
\cline{3-10}          &       & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & \cellcolor[rgb]{ .475,  .678,  .867}0.83 & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & 0.02 \bigstrut\\
    \Xhline{1.1pt}
    \end{tabular}%
     }
  \label{tab:exp2}%
\end{table}%



==> exp3.tex <==
% Table generated by Excel2LaTeX from sheet 'T3'
\begin{table}[htbp]
  \centering
  \caption{The results of Setup 3. Task is Compas-Sex.}
  \vspace{-2ex}
  %\scalebox{0.86}{
  \resizebox{\columnwidth}{!}{
      \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \Xhline{1.1pt}
    \rowcolor[rgb]{ .682,  .667,  .667} \multicolumn{1}{c|}{\textbf{Alg.}} & \textbf{Method} & \textbf{R} & \textbf{P} & \textbf{Acc} & \textbf{F1} & \textbf{AOD} & \textbf{EOD} & \textbf{(M)SPD} \bigstrut\\
    \Xhline{1.1pt}
    \multirow{5}[10]{*}{LR} & Default & \cellcolor[rgb]{ .475,  .678,  .867}0.73 & 0.66  & 0.64  & 0.61  & \cellcolor[rgb]{ .475,  .678,  .867}0.05 & 0.14  & 0.18 \bigstrut\\
\cline{2-9}          & ADV   & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & 0.65  & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & 0.26  & 0.20  & 0.28 \bigstrut\\
\cline{2-9}          & ROC   & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & 0.65  & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & 0.04 \bigstrut\\
\cline{2-9}          & MAAT  & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & 0.67  & \cellcolor[rgb]{ .867,  .922,  .969}0.66 & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & 0.13  & 0.09  & 0.16 \bigstrut\\
\cline{2-9}          & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.72 & \cellcolor[rgb]{ .475,  .678,  .867}0.81 & \cellcolor[rgb]{ .475,  .678,  .867}0.72 & \cellcolor[rgb]{ .475,  .678,  .867}0.72 & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & 0.04 \bigstrut\\
     \Xhline{1.1pt}
    \multirow{5}[10]{*}{RF} & Default & \cellcolor[rgb]{ .475,  .678,  .867}0.75 & \cellcolor[rgb]{ .867,  .922,  .969}0.66 & \cellcolor[rgb]{ .867,  .922,  .969}0.67 & \cellcolor[rgb]{ .475,  .678,  .867}0.72 & 0.11  & 0.18  & 0.2 \bigstrut\\
\cline{2-9}          & ADV   & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & 0.65  & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & 0.65  & 0.26  & 0.20  & 0.28 \bigstrut\\
\cline{2-9}          & ROC   & 0.62  & 0.63  & 0.63  & 0.62  & 0.15  & 0.15  & 0.12 \bigstrut\\
\cline{2-9}          & MAAT  & 0.64  & 0.64  & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & 0.64  & 0.08  & 0.06  & 0.11 \bigstrut\\
\cline{2-9}          & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.71 & \cellcolor[rgb]{ .475,  .678,  .867}0.73 & \cellcolor[rgb]{ .475,  .678,  .867}0.73 & \cellcolor[rgb]{ .475,  .678,  .867}0.71 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & \cellcolor[rgb]{ .475,  .678,  .867}0.05 & 0.04 \bigstrut\\
   \Xhline{1.1pt}
    \multirow{5}[10]{*}{SVM} & Default & \cellcolor[rgb]{ .22,  .525,  .8}0.77 & \cellcolor[rgb]{ .867,  .922,  .969}0.66 & \cellcolor[rgb]{ .867,  .922,  .969}0.67 & \cellcolor[rgb]{ .475,  .678,  .867}0.71 & 0.10  & 0.15  & 0.22 \bigstrut\\
\cline{2-9}          & ADV   & 0.65  & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & 0.26  & 0.20  & 0.28 \bigstrut\\
\cline{2-9}          & ROC   & 0.65  & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & \cellcolor[rgb]{ .867,  .922,  .969}0.65 & \cellcolor[rgb]{ .333,  .592,  .827}0.04 & \cellcolor[rgb]{ .333,  .592,  .827}0.04 & 0.03 \bigstrut\\
\cline{2-9}          & MAAT  & 0.64  & \cellcolor[rgb]{ .867,  .922,  .969}0.66 & \cellcolor[rgb]{ .867,  .922,  .969}0.66 & 0.64  & 0.13  & 0.09  & 0.16 \bigstrut\\
\cline{2-9}          & FITNESS & \cellcolor[rgb]{ .475,  .678,  .867}0.70 & \cellcolor[rgb]{ .475,  .678,  .867}0.73 & \cellcolor[rgb]{ .475,  .678,  .867}0.70 & \cellcolor[rgb]{ .475,  .678,  .867}0.70 & \cellcolor[rgb]{ .475,  .678,  .867}0.03 & \cellcolor[rgb]{ .475,  .678,  .867}0.04 & 0.04 \bigstrut\\
   \Xhline{1.1pt}
    \end{tabular}%
    }
  \label{tab:exp3}%
\end{table}%


==> exp_RQ1_Demo.tex <==
% Table generated by Excel2LaTeX from sheet 'RQ3'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \rowcolor[rgb]{ .988,  .933,  .886} Alg.  & Task  & Method & Acc   & R     & P     & F1    & SPD   & AOD   & EOD \bigstrut\\
    \hline
    \multirow{20}[40]{*}{\begin{turn}{-90}Random Forest\end{turn}} & \multirow{5}[10]{*}{\begin{turn}{-90}Adult-Sex\end{turn}} & Default & \cellcolor[rgb]{ .71,  .827,  .851}0.84 & \cellcolor[rgb]{ .71,  .827,  .851}0.77 & \cellcolor[rgb]{ .71,  .827,  .851}0.80 & \cellcolor[rgb]{ .71,  .827,  .851}0.78 & 0.19  & 0.08  & 0.08 \bigstrut\\
\cline{3-10}          &       & MAAT  & \cellcolor[rgb]{ .435,  .627,  .675}0.85 & \cellcolor[rgb]{ .71,  .827,  .851}0.74 & \cellcolor[rgb]{ .71,  .827,  .851}0.81 & \cellcolor[rgb]{ .71,  .827,  .851}0.77 & 0.13  & \cellcolor[rgb]{ .71,  .827,  .851}0.03 & \cellcolor[rgb]{ .435,  .627,  .675}0.02 \bigstrut\\
\cline{3-10}          &       & Fair SMOTE & \cellcolor[rgb]{ .71,  .827,  .851}0.83 & \cellcolor[rgb]{ .435,  .627,  .675}0.78 & \cellcolor[rgb]{ .71,  .827,  .851}0.78 & \cellcolor[rgb]{ .71,  .827,  .851}0.78 & 0.22  & 0.11  & 0.10 \bigstrut\\
\cline{3-10}          &       & xFAIR & \cellcolor[rgb]{ .71,  .827,  .851}0.83 & 0.52  & 0.69  & 0.59  & \cellcolor[rgb]{ .435,  .627,  .675}0.11 & \cellcolor[rgb]{ .435,  .627,  .675}0.02 & 0.06 \bigstrut\\
\cline{3-10}          &       & FITNESS & \cellcolor[rgb]{ .71,  .827,  .851}0.84 & \cellcolor[rgb]{ .71,  .827,  .851}0.73 & \cellcolor[rgb]{ .71,  .827,  .851}0.81 & \cellcolor[rgb]{ .71,  .827,  .851}0.76 & \cellcolor[rgb]{ .71,  .827,  .851}0.12 & \cellcolor[rgb]{ .71,  .827,  .851}0.03 & \cellcolor[rgb]{ .71,  .827,  .851}0.03 \bigstrut\\
\cline{2-10}          & \multirow{5}[10]{*}{\begin{turn}{-90}Adult-Race\end{turn}} & Default & \cellcolor[rgb]{ .71,  .827,  .851}0.84 & \cellcolor[rgb]{ .71,  .827,  .851}0.77 & \cellcolor[rgb]{ .71,  .827,  .851}0.80 & \cellcolor[rgb]{ .71,  .827,  .851}0.78 & 0.10  & 0.05  & 0.04 \bigstrut\\
\cline{3-10}          &       & MAAT  & \cellcolor[rgb]{ .435,  .627,  .675}0.85 & \cellcolor[rgb]{ .71,  .827,  .851}0.74 & \cellcolor[rgb]{ .71,  .827,  .851}0.81 & \cellcolor[rgb]{ .71,  .827,  .851}0.77 & 0.07  & \cellcolor[rgb]{ .71,  .827,  .851}0.02 & \cellcolor[rgb]{ .71,  .827,  .851}0.03 \bigstrut\\
\cline{3-10}          &       & Fair SMOTE & \cellcolor[rgb]{ .71,  .827,  .851}0.83 & \cellcolor[rgb]{ .435,  .627,  .675}0.78 & \cellcolor[rgb]{ .71,  .827,  .851}0.78 & \cellcolor[rgb]{ .71,  .827,  .851}0.78 & 0.13  & 0.07  & 0.08 \bigstrut\\
\cline{3-10}          &       & xFAIR & \cellcolor[rgb]{ .71,  .827,  .851}0.83 & 0.52  & 0.69  & 0.59  & \cellcolor[rgb]{ .435,  .627,  .675}0.06 & \cellcolor[rgb]{ .435,  .627,  .675}0.00 & \cellcolor[rgb]{ .435,  .627,  .675}0.02 \bigstrut\\
\cline{3-10}          &       & FITNESS & \cellcolor[rgb]{ .71,  .827,  .851}0.84 & \cellcolor[rgb]{ .71,  .827,  .851}0.73 & \cellcolor[rgb]{ .71,  .827,  .851}0.81 & \cellcolor[rgb]{ .71,  .827,  .851}0.76 & \cellcolor[rgb]{ .435,  .627,  .675}0.06 & \cellcolor[rgb]{ .71,  .827,  .851}0.02 & \cellcolor[rgb]{ .71,  .827,  .851}0.03 \bigstrut\\
\cline{2-10}          & \multirow{5}[10]{*}{\begin{turn}{-90}Compas-Sex\end{turn}} & Default & \cellcolor[rgb]{ .435,  .627,  .675}0.65 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & 0.17  & 0.14  & 0.12 \bigstrut\\
\cline{3-10}          &       & MAAT  & \cellcolor[rgb]{ .435,  .627,  .675}0.65 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.65 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & 0.13  & 0.10  & 0.08 \bigstrut\\
\cline{3-10}          &       & Fair SMOTE & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & 0.17  & 0.14  & 0.11 \bigstrut\\
\cline{3-10}          &       & xFAIR & \cellcolor[rgb]{ .435,  .627,  .675}0.65 & \cellcolor[rgb]{ .435,  .627,  .675}0.73 & \cellcolor[rgb]{ .435,  .627,  .675}0.67 & \cellcolor[rgb]{ .435,  .627,  .675}0.70 & \cellcolor[rgb]{ .71,  .827,  .851}0.09 & \cellcolor[rgb]{ .435,  .627,  .675}0.01 & \cellcolor[rgb]{ .71,  .827,  .851}0.05 \bigstrut\\
\cline{3-10}          &       & FITNESS & \cellcolor[rgb]{ .435,  .627,  .675}0.65 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .435,  .627,  .675}0.07 & \cellcolor[rgb]{ .71,  .827,  .851}0.04 & \cellcolor[rgb]{ .71,  .827,  .851}0.04 \bigstrut\\
\cline{2-10}          & \multirow{5}[10]{*}{\begin{turn}{-90}Compas-Race\end{turn}} & Default & \cellcolor[rgb]{ .435,  .627,  .675}0.65 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & 0.14  & 0.12  & 0.09 \bigstrut\\
\cline{3-10}          &       & MAAT  & \cellcolor[rgb]{ .435,  .627,  .675}0.65 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.65 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & 0.11  & 0.09  & \cellcolor[rgb]{ .71,  .827,  .851}0.06 \bigstrut\\
\cline{3-10}          &       & Fair SMOTE & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & 0.12  & 0.10  & 0.07 \bigstrut\\
\cline{3-10}          &       & xFAIR & \cellcolor[rgb]{ .435,  .627,  .675}0.65 & \cellcolor[rgb]{ .435,  .627,  .675}0.73 & \cellcolor[rgb]{ .435,  .627,  .675}0.67 & \cellcolor[rgb]{ .435,  .627,  .675}0.70 & 0.13  & \cellcolor[rgb]{ .435,  .627,  .675}0.02 & 0.09 \bigstrut\\
\cline{3-10}          &       & FITNESS & \cellcolor[rgb]{ .435,  .627,  .675}0.65 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .71,  .827,  .851}0.64 & \cellcolor[rgb]{ .435,  .627,  .675}0.04 & \cellcolor[rgb]{ .71,  .827,  .851}0.04 & \cellcolor[rgb]{ .435,  .627,  .675}0.03 \bigstrut\\
    \hline
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> fig_Intervention.tex <==
\begin{figure}[!t]
%\centering 
\includegraphics[width=0.65\linewidth]{fig/intervention.pdf}
\caption{Causal Intervention}
\label{fig:Causal Intervention} 
\end{figure} 

==> fig_SCM.tex <==
\begin{figure}[!h]
%\centering 
\includegraphics[width=0.5\linewidth]{fig/casualeg1.pdf}
\caption{Causal Graph}
\label{fig:SCM} 
\end{figure} 
